Structure and Topology of Band Structures in the 1651 Magnetic Space Groups

The properties of electrons in magnetically ordered crystals are of interest both from the viewpoint of realizing novel topological phases, such as magnetic Weyl semimetals, and from the applications perspective of creating energy-efficient memories. A systematic study of symmetry and topology in magnetic materials has been challenging given that there are 1651 magnetic space groups (MSGs). Here, by using an efficient representation of allowed band structures, we obtain a systematic description of several basic properties of free electrons in all MSGs in three dimensions as well as in the 528 magnetic layer groups relevant to two dimensional magnetic materials. We compute constraints on electron fillings and band connectivity compatible with insulating behavior. Also, by contrasting with atomic insulators, we identify band topology entailed by the symmetry transformation of bands, as determined by the MSG alone. We give an application of our results to identifying topological semimetals arising in periodic arrangements of hedgehog-like magnetic textures.

==> spinful_Hexa2_foot.tex <==
\newlength{\tabLspinfulHexa2} 
\settowidth{\tabLspinfulHexa2}{\input{spinful_Hexa2}} 
\begin{minipage}{\tabLspinfulHexa2} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinful_Hexa_foot.tex <==
\newlength{\tabLspinfulHexa} 
\settowidth{\tabLspinfulHexa}{\input{spinful_Hexa}} 
\begin{minipage}{\tabLspinfulHexa} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }
\end{flushleft}\end{minipage}

==> spinful_MLGII_foot.tex <==
\newlength{\tabLspinfulMLGII} 
\settowidth{\tabLspinfulMLGII}{\input{spinful_MLGII}} 
\begin{minipage}{\tabLspinfulMLGII} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ }
\end{flushleft}
\end{minipage}

==> spinful_MLG_foot.tex <==
\newlength{\tabLspinfulMLG} 
\settowidth{\tabLspinfulMLG}{\input{spinful_MLG}} 
\begin{minipage}{\tabLspinfulMLG} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ }
\end{flushleft}
\end{minipage}

==> spinful_Ortho2_foot.tex <==
\newlength{\tabLspinfulOrtho2} 
\settowidth{\tabLspinfulOrtho2}{\input{spinful_Ortho2}} 
\begin{minipage}{\tabLspinfulOrtho2} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinful_Ortho3_foot.tex <==
\newlength{\tabLspinfulOrtho3} 
\settowidth{\tabLspinfulOrtho3}{\input{spinful_Ortho3}} 
\begin{minipage}{\tabLspinfulOrtho3} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinful_OrthoII_foot.tex <==
\newlength{\tabLspinfulOrthoII} 
\settowidth{\tabLspinfulOrthoII}{\input{spinful_OrthoII}} 
\begin{minipage}{\tabLspinfulOrthoII} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }
\end{flushleft}\end{minipage}

==> spinful_Ortho_foot.tex <==
\newlength{\tabLspinfulOrtho} 
\settowidth{\tabLspinfulOrtho}{\input{spinful_Ortho}} 
\begin{minipage}{\tabLspinfulOrtho} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }
\end{flushleft}\end{minipage}

==> spinful_Tetra2_foot.tex <==
\newlength{\tabLspinfulTetra2} 
\settowidth{\tabLspinfulTetra2}{\input{spinful_Tetra2}} 
\begin{minipage}{\tabLspinfulTetra2} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinful_Tetra3_foot.tex <==
\newlength{\tabLspinfulTetra3} 
\settowidth{\tabLspinfulTetra3}{\input{spinful_Tetra3}} 
\begin{minipage}{\tabLspinfulTetra3} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinful_TetraII_foot.tex <==
\newlength{\tabLspinfulTetraII} 
\settowidth{\tabLspinfulTetraII}{\input{spinful_TetraII}} 
\begin{minipage}{\tabLspinfulTetraII} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }
\end{flushleft}\end{minipage}

==> spinful_Tetra_foot.tex <==
\newlength{\tabLspinfulTetra} 
\settowidth{\tabLspinfulTetra}{\input{spinful_Tetra}} 
\begin{minipage}{\tabLspinfulTetra} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }
\end{flushleft}\end{minipage}

==> spinless_Hexa2_foot.tex <==
\newlength{\tabLspinlessHexa2} 
\settowidth{\tabLspinlessHexa2}{\input{spinless_Hexa2}} 
\begin{minipage}{\tabLspinlessHexa2} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinless_Hexa_foot.tex <==
\newlength{\tabLspinlessHexa} 
\settowidth{\tabLspinlessHexa}{\input{spinless_Hexa}} 
\begin{minipage}{\tabLspinlessHexa} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }
\end{flushleft}\end{minipage}

==> spinless_Ortho2_foot.tex <==
\newlength{\tabLspinlessOrtho2} 
\settowidth{\tabLspinlessOrtho2}{\input{spinless_Ortho2}} 
\begin{minipage}{\tabLspinlessOrtho2} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinless_Ortho3_foot.tex <==
\newlength{\tabLspinlessOrtho3} 
\settowidth{\tabLspinlessOrtho3}{\input{spinless_Ortho3}} 
\begin{minipage}{\tabLspinlessOrtho3} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinless_OrthoII_foot.tex <==
\newlength{\tabLspinlessOrthoII} 
\settowidth{\tabLspinlessOrthoII}{\input{spinless_OrthoII}} 
\begin{minipage}{\tabLspinlessOrthoII} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }\\ 
$*$: Exhibiting exceptional filling pattern; see Table \ref{tab:spinlessnuEx} 
\end{flushleft}\end{minipage}

==> spinless_Ortho_foot.tex <==
\newlength{\tabLspinlessOrtho} 
\settowidth{\tabLspinlessOrtho}{\input{spinless_Ortho}} 
\begin{minipage}{\tabLspinlessOrtho} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }\\ 
$*$: Exhibiting exceptional filling pattern; see Table \ref{tab:spinlessnuEx} 
\end{flushleft}\end{minipage}

==> spinless_Tetra2_foot.tex <==
\newlength{\tabLspinlessTetra2} 
\settowidth{\tabLspinlessTetra2}{\input{spinless_Tetra2}} 
\begin{minipage}{\tabLspinlessTetra2} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinless_Tetra3_foot.tex <==
\newlength{\tabLspinlessTetra3} 
\settowidth{\tabLspinlessTetra3}{\input{spinless_Tetra3}} 
\begin{minipage}{\tabLspinlessTetra3} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$ \\ 
$X_{\rm BS}$:Symmetry-based indicators of band topology \\ 
$\nu_{\rm BS}$:Set of $\nu$ bands can only be isolated by band gaps if $\nu \in \nu_{\rm BS}\, \mathbb Z$ } 
\end{flushleft}\end{minipage}

==> spinless_TetraII_foot.tex <==
\newlength{\tabLspinlessTetraII} 
\settowidth{\tabLspinlessTetraII}{\input{spinless_TetraII}} 
\begin{minipage}{\tabLspinlessTetraII} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }\\ 
$*$: Exhibiting exceptional filling pattern; see Table \ref{tab:spinlessnuEx} 
\end{flushleft}\end{minipage}

==> spinless_Tetra_foot.tex <==
\newlength{\tabLspinlessTetra} 
\settowidth{\tabLspinlessTetra}{\input{spinless_Tetra}} 
\begin{minipage}{\tabLspinlessTetra} 
\begin{flushleft} 
{\footnotesize $d$: Rank of the band structure group $\{{\rm BS}\}$\\ 
$X_{\rm BS}$: Symmetry-based indicators of band topology\\ 
$\nu_{\rm BS}$: Set of $\nu$ bands are symmetry-forbidden from being isolated by band gaps if $\nu \not \in \nu_{\rm BS}\, \mathbb Z$ }\\ 
$*$: Exhibiting exceptional filling pattern; see Table \ref{tab:spinlessnuEx} 
\end{flushleft}\end{minipage}
